Shedding a PAC-Bayesian Light on Adaptive Sliced-Wasserstein Distances

The Sliced-Wasserstein distance (SW) is a computationally efficient and theoretically grounded alternative to the Wasserstein distance. Yet, the literature on its statistical properties -- or, more accurately, its generalization properties -- with respect to the distribution of slices, beyond the uniform measure, is scarce. To bring new contributions to this line of research, we leverage the PAC-Bayesian theory and a central observation that SW may be interpreted as an average risk, the quantity PAC-Bayesian bounds have been designed to characterize. We provide three types of results: i) PAC-Bayesian generalization bounds that hold on what we refer as adaptive Sliced-Wasserstein distances, i.e. SW defined with respect to arbitrary distributions of slices (among which data-dependent distributions), ii) a principled procedure to learn the distribution of slices that yields maximally discriminative SW, by optimizing our theoretical bounds, and iii) empirical illustrations of our theoretical findings.

==> expe_gen_model.tex <==
\newpage

\subsubsection{Illustrating generalization properties on generative modelling}

For evaluating the generalization property of our distance in a MNIST  generative modelling context, we have compared the performance of a generative model trained using 
a distributional SW distance as a loss. For DSW, the distribution of the slices is learned
at every minibatch of data, and in our case we evaluate the robustness and generalization ability of the learned distribution  by learning it only every 
$10$ or $50$ minibatches. We make the hypothesis that if the learned distribution generalizes well to unseen datasets, then gradient obtained from the distance between
minibatches would still provide sufficient information to learn the generative model.

For training the model, we followed the same approach (architecture and optimizer) as the one described in \cite{nguyen2021distributional}. For each minibatch of size $512$, the distribution $\rho$ is learned by optimizing $100$ push-forwarded projections over $100$ iterations while the generative model is
trained over $400$ epochs. For a sake of comparison, we report also results of a generative model trained with maxSW.

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
\includegraphics[width=7cm]{./figure/genmodel_wd.png}    \caption{Evolution of the Wasserstein distance between a set of generated MNIST digits and the true MNIST test set with respect to training time. 
%Each curve is obtained for a specific Sliced distance and for different update rate of the distribution $\rho$. DSWD, DSWD-10 and DSWD-50 refees respectively to a distributional SWD where the distribution of the slices are learnet at every minibatch, every 10 minibatch and every 50 minibatch. Similarly maxSWD and maxSWD-10 refers to optimizing for the max slice every minibatch and every 10 minibatches.
}
    \label{fig:genmodevolution}
\end{wrapfigure}


Figure \ref{fig:genmodevolution} shows the evolution of the Wasserstein distance between generated MNIST and MNIST test set with respects to running time of training (measured after each epoch).
 Each curve is obtained for a specific Sliced distance and for different update rate of the distribution $\rho$. DSW, DSW-10 and DSW-50 refer respectively to a distributional SW distance where the distribution of the slices are learned at every minibatch, every 10 minibatch and every 50 minibatch. Similarly maxSW and maxSW-10 refers to optimizing for the max slice every minibatch and every 10 minibatch.
We can see from these plots that the
classical distributional Sliced Wasserstein yields a WD of about 29 after approximately $10^4$ seconds. When learning the distribution of slices only every $10$ minibatch, we achieve similar WD value (30) with a twice less running time. When further reducing the
frequency of updating the distribution (DSWD-50), we converge faster at the expense for
further loss in quality of generation (WD~34). Our result on maxSW confirms our theoretical
analysis in the sense that, as for many learning problem, regularization is key and
allows to generalize on unseen data. Indeed, we can see that, while using maxSW as a loss yields to generative model with a reasonable performance, optimizing the max slice only every $10$ minibatch leads to a very unstable learning and poorer performances. Examples of generated digits are also presented in the appendix.

\begin{figure}
    \centering
    ~\hfill
    \includegraphics[width=3cm]{./figure/dswd-1-sample_epoch_399.png}
    ~\hfill~
    \includegraphics[width=3cm]{./figure/dswd-10-sample_epoch_399.png}
    ~\hfill~
    \includegraphics[width=3cm]{./figure/max-1-sample_epoch_399.png}
    ~\hfill~
    \includegraphics[width=3cm]{./figure/max-10-sample_epoch_399.png}
    \hfill~
    \caption{Examples of generated MNIST digits. From left to right : DSWD, DSWD with update of $\rho$ every $10$ minibatch, maxSWD, maxSWD with update of $\rho$ every $10$ minibatch.}
    \label{fig:my_label}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

